Geometry-Based Grasping of Vine Tomatoes

We propose a geometry-based grasping method for vine tomatoes. It relies on a computer-vision pipeline to identify the required geometric features of the tomatoes and of the truss stem. The grasping method then uses a geometric model of the robotic hand and the truss to determine a suitable grasping location on the stem. This approach allows for grasping tomato trusses without requiring delicate contact sensors or complex mechanistic models and under minimal risk of damaging the tomatoes. Lab experiments were conducted to validate the proposed methods, using an RGB-D camera and a low-cost robotic manipulator. The success rate was 83% to 92%, depending on the type of truss.

==> glossary.tex <==
\newacronym{hsv}{HSV}{hue, saturation and value}
\newacronym{hsi}{HSI}{hue, saturation and intensity}
\newacronym{hsl}{HSL}{hue, saturation and lightness}
\newacronym{rgb}{RGB}{red, green and blue}
\newacronym{ir}{IR}{infra red}

\newacronym{pca}{PCA}{principle component analysis}	
\newacronym{ransac}{RANSAC}{Random sample consensus}
\newacronym{cht}{CHT}{Circle Hough Transform}

\newacronym{ros}{ROS}{Robot Operating System}


% === Geometric model ===
\nomenclature[G]{$r_i$}{Tomato radius}
\nomenclature[G]{$\vec{c}_i$}{Tomato center}
\nomenclature[G]{$w$}{end effector width}
\nomenclature[G]{$h_{\text{tip}}$}{fingertip height}
\nomenclature[G]{$t_\text{{tip}}$}{fingertip thickness}
\nomenclature[G]{$d_{\text{tip}}$}{controllable distance between end effector fingers}
\nomenclature[G]{$l$}{end effector length}


% === Experimental Results ===
\nomenclature[G]{TP}{The number of true positive predictions}
\nomenclature[G]{FP}{The number of false positive predictions}
\nomenclature[G]{FN}{The number of false negative predictions}
\nomenclature[G]{TPR}{The true positive rate}
\nomenclature[G]{FDR}{The false discovery rate}

\nomenclature[G]{$L$}{Distance threshold from the junctions encapsulating the branch}
\nomenclature[G]{$c$}{safety factor}.
\nomenclature[G]{$\alpha$}{Peduncle curvature threshold}
\nomenclature[G]{$l_\text{min}$}{Minimum branch length in millimeter}

\nomenclature[G]{$c_\text{fill}$}{minimum required overlap between candidate circle and tomato segment}

%% This code creates the groups
% -----------------------------------------
\renewcommand\nomgroup[1]{%
  \item[\bfseries
  \ifstrequal{#1}{G}{Geometric Model Parameters}{%
  \ifstrequal{#1}{N}{Number Sets}{%
  \ifstrequal{#1}{O}{Other Symbols}{}}}%
]}
% -----------------------------------------

==> misc/failure_rate.tex <==
\section{Experiments}
\label{sec:experiments}
Real-world experiments were conducted to validate the proposed geometry-based grasping method for vine tomato. These experiments were performed in a well controlled lab environment.

\subsection{Experimental Setup}
The physical setup consists of a robotic manipulator, an RGB-D vision system and several tomato trusses as shown in Figure~\ref{fig:05:setup:a}. The five degree of freedom Interbotix PincherX 150 Robot Arm offers a maximum working payload of 50g\footnote{\url{https://www.trossenrobotics.com/pincherx-150-robot-arm.aspx}}. The gripper fingers are covered with deformable foam as required for the soft-part caging condition. Furthermore, rubber knobs were attached to these fingers such that they can enclose the peduncle. The end effector is shown in a open configuration in Figure~\ref{fig:05:setup:b}.

\begin{figure}[htb]
    \begin{subfigure}[t]{0.6\linewidth}
        \centering
	    \includegraphics[height = 3cm]{05/setup.jpeg}
	    \caption{An overview of the experimental setup.}
	    \label{fig:05:setup:a}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.35\linewidth}
	    \centering
	    \includegraphics[height = 3cm]{05/ee_open.jpg}
	    \caption{The custom end effector.}
	    \label{fig:05:setup:b}
	\end{subfigure}
	% \caption{Experimental setup}
	\label{fig:05:setup}
\end{figure}

The Intel RealSense Depth Camera D435\footnote{\url{https://www.intelrealsense.com/depth-camera-d435/}} is used which combines active \acrlong{ir} stereo technology to measure depth with an RGB sensor for color information. Since a sense-plan-act framework is used, the camera is placed in an eye-on-base configuration. The camera in unable to obtain accurate depth information about the peduncle. Hence, the peduncle height is taken as a constant measured before conducting an experiment.

\todo[inline]{Think about what truss stems to use for the realistic model, maybe redo some experiments?}
Plastic tomato models are used since payload limitations do not allow for executing pick and place tasks on real tomato trusses. Six truss models of two different categories are created: 
\begin{enumerate}
	\item \textbf{Simple truss}: artificial tomatoes are attached to an artificial stem. The peduncle has a large diameter and a simple straight shape. % Three models were created as shown in Figure~\ref{fig:05:target:a} to \ref{fig:05:target:c}.
	\item \textbf{Realistic truss}: artificial tomatoes are attached to a real stem. Truss stems with sufficient space around the peduncle to fit the gripper fingers were selected. % Trusses of various shapes were created, as shown in Figure~\ref{fig:05:target:d} to \ref{fig:05:target:f}.
\end{enumerate} 

\iffalse
\begin{figure}[htbp]
	\centering
	\begin{subfigure}[t]{0.3\textwidth}
	    \vskip 0pt
		\centering
		\includegraphics[width = \linewidth]{05/model/001.jpg}
		\caption{Simple truss model 1}
		\label{fig:05:target:a}
	\end{subfigure}		
	\begin{subfigure}[t]{0.3\textwidth}
	    \vskip 0pt
		\centering
		\includegraphics[width = \linewidth]{05/model/002.jpg}
		\caption{Simple truss model 2}
		\label{fig:05:target:b}
	\end{subfigure}	
	\begin{subfigure}[t]{0.3\textwidth}
	    \vskip 0pt
		\centering
		\includegraphics[width = \linewidth]{05/model/003.jpg}
		\caption{Simple truss model 3}
		\label{fig:05:target:c}
	\end{subfigure}	
	
	\begin{subfigure}[t]{0.3\textwidth}
	    \vskip 0pt
		\centering
		\includegraphics[width = \linewidth]{05/model/004.jpg}
		\caption{Realistic truss model 1}
		\label{fig:05:target:d}
	\end{subfigure}	
	\begin{subfigure}[t]{0.3\textwidth}
	    \vskip 0pt
		\centering
		\includegraphics[width = \linewidth]{05/model/005.jpg}
		\caption{Realistic truss model 2}
		\label{fig:05:target:e}
	\end{subfigure}	
	\begin{subfigure}[t]{0.3\textwidth}
	    \vskip 0pt
		\centering
		\includegraphics[width = \linewidth]{05/model/006.jpg}
		\caption{Realistic truss model 3}
		\label{fig:05:target:f}
	\end{subfigure}	
	\caption{Overview of the truss models used for the pick and place routines.}
	\label{fig:05:target}
\end{figure}
\fi

\subsection{Task}
A pick and place routine is executed to determine the strengths and weaknesses of this method. The task consists of five successive parts: (i) the truss is detected and relevant features are extracted, (ii) the end effector moves towards and wraps around the peduncle, (iii) the truss is lifted off the supporting surface, (iv) the truss is moved to an arbitrary target pose, and (v) the truss is placed back on the supporting surface. This task is successful if all these parts are completed. The following modes of failure may be observed:
\begin{itemize}
	\item \textbf{Vision}: the vision system fails to identify key features required for the geometric model, such as the peduncle, or junctions. These failures are caused by the computer vision pipeline.
	\item \textbf{Planning}:  the grasp planning algorithm fails to determine a valid grasp action. For example, a pose which can not be reached by the end-effector due to space constraints. This error shows weaknesses in the geometry-based grasping method.
	\item \textbf{Control}: the manipulator fails to execute the planned task. A typical example is the end effector not reaching the target pose. These errors show weaknesses in the used hardware, calibration, and implementation such as used filters.
	\item \textbf{Overload}: the hardware fails to execute the task at hand due to overloading or overheating of the servo motors.
\end{itemize}
In case the task is not successfully executed, the mode of failure will be noted for later discussion. Since the goal of this experiment is not to test the load capacities of the robot, overload failures will be ignored. When a grasp fails the truss is moved to a new random pose by the human operator such that the experiment can continue.



\subsection{Results}
\label{sec:05:results}
The previously described pick and place routine is performed 20 times per truss, such that the truss needs to be grasped from several different poses. The failure rates are provided in Table~\ref{tab:results}, some grasps are shown in Figure~\ref{fig:06:result}. Videos taken during the experiment can be found via SurfDrive\footnote{\url{https://surfdrive.surf.nl/files/index.php/s/euEKKhtSRqB9mPG}}. 

\begin{table}[htb]
	\centering
	\caption{Failure rates of the proposed geometry-based grasping method applied to various truss models. Two different model categories were used. The simple models use an artificial stem, whereas the realistic models consist of a real vine tomato stem.}
	\label{tab:results}
	\begin{tabular}{m{0.2cm} l m{1cm}  l| l | l l l} 
							&			&			&			& \multicolumn{4}{c}{failure rate (failures)}\\
					& \multicolumn{2}{l}{model id}  & attempts	& all 	&vision 	& 
		planning & control 	\\ \hline
		\multirow{4}{*}{\rotatebox[origin=c]{90}{simple}}  	
	    & \textbf{all}	&\includegraphics[height = 0.6cm]{fig/height.png} & \textbf{60}		& \textbf{8\% (5)}	& \textbf{3\% (2)}	& \textbf{3\% (2)}		& \textbf{2\% (1)}	\\
		  					& 1	& \includegraphics[height = 0.6cm]{fig/05/model/001.jpg}		& 20		& 5\% (1)	& 5\% (1)	& 0\% (0)		& 0\% (0)	\\
		  					& 2	& \includegraphics[height = 0.6cm]{fig/05/model/002.jpg}		& 20		& 20\% (4)	& 5\% (1)	& 10\% (2)		& 5\% (1)	\\ 
		  					& 3	& \includegraphics[height = 0.6cm]{fig/05/model/003.jpg}		& 20		& 0\% (0)	& 0\% (0)	& 0\% (0)		& 0\% (0)	\\ \hline

		\multirow{4}{*}{\rotatebox[origin=c]{90}{realistic}}  & \textbf{all}    & \includegraphics[height = 0.6cm]{fig/height.png}		& \textbf{60}		& \textbf{17\% (10)}	& \textbf{0\% (0)}	& \textbf{7\% (4)}		& \textbf{10\% (6)}	\\ 
							& 1	& \includegraphics[height = 0.6cm]{fig/05/model/004.jpg}		& 20		& 0\% (0)	& 0\% (0)	& 0\% (0)		& 0\% (0)	\\
							& 2	& \includegraphics[height = 0.6cm]{fig/05/model/005.jpg}		& 20		&25\% (5)	& 0\% (0)	& 20\% (4)		& 5\% (1)	\\
							& 3	& \includegraphics[height = 0.6cm]{fig/05/model/006.jpg}		& 20		&25\% (5)	& 0\% (0)	& 0\% (0)		& 25\% (5)	\\
	\end{tabular}
\end{table}

% simple
A failure rate of 8\% (5/60) was obtained on the simple models. A typical successful grasp is shown in Figure~\ref{fig:06:result:a}. From the five failures, two were caused by vision, two by planning, and a single failure was caused by control.
%
For both vision failures, the algorithm was unable to identify the peduncle.
%
In both planning errors, the algorithm did not take into account the surrounding pedicels, causing the end effector to be blocked. An example is shown in Figure \ref{fig:06:result:b}.
%
The other failure was caused by control, where the end effector closed above the peduncle. Most failures occurred on model two, a single failure was made on model one, and no failures were made on model three. Undesired tilting of the second model was frequently observed as shown in Figure \ref{fig:06:result:c}.

\begin{figure}[hp]
 	\centering
 	\begin{subfigure}[t]{\textwidth}
 		\centering
 		\includegraphics[height=4cm]{05/010.png}
 		\hfill
 		\includegraphics[height=4cm]{05/success.png}
 		\caption{A successful grasp where the end effector fingers wrap around the peduncle.}
 		\label{fig:06:result:a}
 	\end{subfigure}	
 	\vfill
 	\begin{subfigure}[t]{\textwidth}
 		\centering
 		\includegraphics[height=4cm]{05/009.png}
 		\hfill
 		\includegraphics[height=4cm]{05/failure.png}
 		\caption{A failed grasp where the planned closing actions causes the end effector fingers to get stuck on the pedicel.}
 		\label{fig:06:result:b}
 	\end{subfigure}		
 	\vfill
 	\begin{subfigure}[t]{\textwidth}
 		\centering
 		\includegraphics[height=4cm]{05/002.png}
 		\hfill
 		\includegraphics[height=4cm]{05/tilt.png}
 		\caption{The model tilts during a grasp.}
 		\label{fig:06:result:c}
 	\end{subfigure}	
  	\caption{A pick and place routine executed on simple truss model two. The left column shows the planned grasp, and the right column shows the grasp applied to the truss. The tomatoes are represented by the dashed circles ($\protect\tomcirc$), the peduncle by the dark green line ($\protect\pendline$), the junctions by the purple dots ($\protect\junccirc$) the center of mass by the crossed circle ($\protect\centerofmass$), and the opened end effector fingers by the orange boxes ($\protect\eebox$), which will be close along the purple lines ($\protect\grasplines$).}
 	\label{fig:06:result}
 \end{figure}
 
 % realistic
On the realistic models, a failure rate of 17\% (10/60) was obtained. Twice as many failures were reported compared to the simple models.
%
All ten failures were caused by pedicels blocking the end effector. Four of these cases were caused by planning, and six cases were the result of control. No failures were caused by the computer vision system.
% 
All grasp attempts on the first model succeeded, an equal number of failures was observed for model two and three. Most failures on model two were caused by planning, on model three control errors occurred more frequently. 
 
 \iffalse
 
 \begin{table}[htbp]
	\centering
	\caption{Failure rates of the proposed geometry-based grasping method applied to various truss models. Two different model categories were used. The simple models use an artificial stem, whereas the realistic models consist of a real vine tomato stem.}
	\label{tab:results}
	\begin{tabular}{l l  l| l | l l l} 
							&			&			&			\multicolumn{4}{c}{failure rate}\\
		category			& model id	& attempts	& all 	&vision 	& planning 		& control 	\\ \hline
		\multirow{4}{*}{simple}  	& \textbf{all}	& \textbf{60}		& \textbf{8\% (5)}	& \textbf{3\% (2)}	& \textbf{3\% (2)}		& \textbf{2\% (1)}	\\ 		
		  					& 1			& 20		& 5\% (1)	& 5\% (1)	& 0\% (0)		& 0\% (0)	\\ 		
		  					& 2			& 20		& 20\% (4)	& 5\% (1)	& 10\% (2)		& 5\% (1)	\\ 
		  					& 3			& 20		& 0\% (0)	& 0\% (0)	& 0\% (0)		& 0\% (0)	\\ \hline

		\multirow{4}{*}{realistic}  & \textbf{all}		& \textbf{60}		& \textbf{17\% (10)}	& \textbf{0\% (0)}	& \textbf{7\% (4)}		& \textbf{10\% (6)}	\\ 
							& 1			& 20		& 0\% (0)	& 0\% (0)	& 0\% (0)		& 0\% (0)	\\
							& 2			& 20		&25\% (5)	& 0\% (0)	& 20\% (4)		& 5\% (1)	\\
							& 3			& 20		&25\% (5)	& 0\% (0)	& 0\% (0)		& 25\% (5)	\\
	\end{tabular}
\end{table}

\fi
